[Re] Pure Noise to the Rescue of Insufficient Data

We examine the main claims of Zada, Benou, and Irani (2021), which states that in an image classification task with imbalanced training data, (i) using pure noise to augment minority-class images encourages generalization by improving minority-class accuracy. This method is paired with (ii) a new batch normalization layer that normalizes noise images using affine parameters learned from natural images, which improves the model's performance. Moreover, (iii) this improvement is robust to varying levels of data augmentation. Finally, the authors propose that (iv) adding pure noise images can improve classification even on balanced training data. We implemented the training pipeline from the description of the paper using PyTorch and integrated authors' code snippets for sampling pure noise images and batch normalizing noise and natural images separately. We reproduced the main claims that (i) oversampling with pure noise improves generalization by improving the minority-class accuracy, (ii) the proposed batch normalization (BN) method outperforms baselines, (iii) and this improvement is robust across data augmentations. Our results also support that (iv) adding pure noise images can improve classification on balanced training data. However, additional experiments suggest that the performance improvement from OPeN may be more orthogonal to the improvement caused by a bigger network or more complex data augmentation.

==> metadata.tex <==
% DO NOT EDIT - automatically generated from metadata.yaml

\def \codeURL{https://github.com/seungjaeryanlee/pure-noise}
\def \codeDOI{10.5281/zenodo.7947264}
\def \codeSWH{swh:1:dir:41b1ddbd87720da65e78d56dfc86b8eb81dbba56}
\def \dataURL{}
\def \dataDOI{}
\def \editorNAME{Koustuv Sinha,\\ Maurits Bleeker,\\ Samarth Bhargav}
\def \editorORCID{}
\def \reviewerINAME{}
\def \reviewerIORCID{}
\def \reviewerIINAME{}
\def \reviewerIIORCID{}
\def \dateRECEIVED{04 February 2023}
\def \dateACCEPTED{19 April 2023}
\def \datePUBLISHED{20 July 2023}
\def \articleTITLE{[Re] Pure Noise to the Rescue of Insufficient Data}
\def \articleTYPE{Replication}
\def \articleDOMAIN{ML Reproducibility Challenge 2022}
\def \articleBIBLIOGRAPHY{bibliography.bib}
\def \articleYEAR{2023}
\def \reviewURL{https://openreview.net/forum?id=ErBe4MnsVD}
\def \articleABSTRACT{We examine the main claims of the original paper [1], which states that in an image classification task with imbalanced training data, (i) using pure noise to augment minority‐class images encourages generalization by improving minority-class accuracy. This method is paired with (ii) a new batch normalization layer that normalizes noise images using affine parameters learned from natural images, which improves the model’s performance. Moreover, (iii) this improvement is robust to varying levels of data augmentation. Finally, the authors propose that (iv) adding pure noise images can improve classification even on balanced training data.}
\def \replicationCITE{S. Zada, I. Benou, and M. Irani. “Pure Noise to the Rescue of Insufficient Data: Improving Imbalanced Classification by Training on Random Noise Images.” In: CoRR abs/2112.08810 (2021). arXiv: 2112.08810.}
\def \replicationBIB{PureNoise}
\def \replicationURL{https://arxiv.org/pdf/2112.08810.pdf}
\def \replicationDOI{}
\def \contactNAME{Seungjae Ryan Lee}
\def \contactEMAIL{ry@nlee.ai}
\def \articleKEYWORDS{rescience c, rescience x, python, pytorch, wandb, machine learning, deep learning}
\def \journalNAME{ReScience C}
\def \journalVOLUME{9}
\def \journalISSUE{2}
\def \articleNUMBER{45}
\def \articleDOI{10.5281/zenodo.8173763}
\def \authorsFULL{Seungjae Ryan Lee and Seungmin Brian Lee}
\def \authorsABBRV{S.R. Lee and S.B. Lee}
\def \authorsSHORT{Lee and Lee}
\title{\articleTITLE}
\date{}
\author[1,\orcid{0000-0002-4589-8892}]{Seungjae Ryan Lee}
\author[2,\orcid{0009-0006-7562-6886}]{Seungmin Brian Lee}
\affil[1]{Bloomberg LP, New York, NY, United States}
\affil[2]{Independent}

